Unimodal Mono-Partite Matching in a Bandit Setting

We tackle a new emerging problem, which is finding an optimal monopartite matching in a weighted graph. The semi-bandit version, where a full matching is sampled at each iteration, has been addressed by \cite{ADMA}, creating an algorithm with an expected regret matching $O(\frac{L\log(L)}{\Delta}\log(T))$ with $2L$ players, $T$ iterations and a minimum reward gap $\Delta$. We reduce this bound in two steps. First, as in \cite{GRAB} and \cite{UniRank} we use the unimodality property of the expected reward on the appropriate graph to design an algorithm with a regret in $O(L\frac{1}{\Delta}\log(T))$. Secondly, we show that by moving the focus towards the main question `\emph{Is user $i$ better than user $j$?}' this regret becomes $O(L\frac{\Delta}{\tilde{\Delta}^2}\log(T))$, where $\Tilde{\Delta} > \Delta$ derives from a better way of comparing users. Some experimental results finally show these theoretical results are corroborated in practice.

==> macros.tex <==

%\usepackage[colorinlistoftodos, textwidth=2cm]{todonotes}
%\setlength{\marginparwidth}{1.5cm} % to handle double column

\definecolor{orange}{rgb}{1.0, 0.5, 0.0}
\definecolor{darkgreen}{rgb}{0.0, 0.5, 0.2}


%\newcommand{\commentrg}[1]{{\color{green}Romaric: #1}}
%\newcommand{\commentmr}[1]{{\color{red}Matthieu: #1}}
\newcommand{\commentrg}[2][noinline]{{\todo[color=green, fancyline, #1]{Rom: #2}}}
\newcommand{\commentmr}[2][noinline]{{\todo[color=orange, #1]{Mat: #2}}}

\renewcommand{\commentrg}[2][noinline]{}
\renewcommand{\commentmr}[2][noinline]{}

\newcommand{\newtext}[1]{{\color{blue}#1}}


\RequirePackage{amsthm}
\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{assumption}{Assumption}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
\newtheoremstyle{external}{}{}{\itshape}{}{\bfseries}{.}{.5em}{#1 2}
\theoremstyle{external}
\newtheorem{externallemma}{Lemma}
\newtheoremstyle{named}{}{}{\itshape}{}{\bfseries}{.}{.5em}{\thmnote{#3's }#1}
\theoremstyle{named}
\newtheorem*{namedtheorem}{Theorem}
\newtheorem*{namedlemma}{Lemma}
\newenvironment{sproof}{%
\renewcommand{\proofname}{Sketch of Proof}\proof}{\endproof}

\newcommand{\ouralgo}{{GRAB}}
\newcommand{\ouralgova}{{GRAB}}
\newcommand{\ouralgovb}{{GRAB$^+$}}

\newcommand{\ouralgofullva}{{Nom à trouver v1}}
\newcommand{\ouralgofullvb}{{Nom à trouver v2}}

\newcommand{\NtR}{{Set}}

\newcommand{\ouralgolong}{{parametric Graph for unimodal RAnking Bandit}}
\newcommand{\ouralgofull}{{S-GRAB}}
\newcommand{\ouralgofulllong}{{Static Graph for unimodal RAnking Bandit}}
\newcommand{\ourmodel}{{MM}}
\newcommand{\ourstrictmodel}{{sMM}}

\newcommand{\mapping}{{\cal F}}
\newcommand{\GG}{{G_\text{rank}}}
\newcommand{\lGG}{{G_\text{lrank}}}


\newcommand{\muh}[1]{\sum_\ell\hat\rho_{#1_\ell,\ell}(t)}


\usepackage{tikz}
%\usepackage[customcolors]{hf-tikz}
%\usetikzlibrary{positioning}
\usetikzlibrary{shapes}
%\usetikzlibrary{shapes, shapes.misc, backgrounds}
%\usetikzlibrary{calc}
%\usetikzlibrary{decorations.pathreplacing}



==> macros_math.tex <==
\RequirePackage{amsmath, amssymb, mathrsfs, bm, dsfont}

\newcommand{\vect}[1]{{\pmb{#1}}} % vector in bold
\newcommand{\av}{\vect{a}}
\newcommand{\bv}{\vect{b}}
\newcommand{\cv}{\vect{c}}
\newcommand{\dv}{\vect{d}}
\newcommand{\ev}{\vect{e}}
\newcommand{\fv}{\vect{f}}
\newcommand{\gv}{\vect{g}}
\newcommand{\hv}{\vect{h}}
\newcommand{\iv}{\vect{i}}
\newcommand{\jv}{\vect{j}}
\newcommand{\kv}{\vect{k}}
\newcommand{\lv}{\vect{l}}
\newcommand{\mv}{\vect{m}}
\newcommand{\nv}{\vect{n}}
\newcommand{\ov}{\vect{o}}
\newcommand{\pv}{\vect{p}}
\newcommand{\qv}{\vect{q}}
\newcommand{\rv}{\vect{r}}
\newcommand{\sv}{\vect{s}}
\newcommand{\tv}{\vect{t}}
\newcommand{\uv}{\vect{u}}
\newcommand{\vv}{\vect{v}}
\newcommand{\wv}{\vect{w}}
\newcommand{\xv}{\vect{x}}
\newcommand{\yv}{\vect{y}}
\newcommand{\zv}{\vect{z}}
\newcommand{\ellv}{\vect{\ell}}

\newcommand{\onev}{{\pmb{1}}}
\newcommand{\alphav}{{\pmb{\alpha}}}
\newcommand{\betav}{{\pmb{\beta}}}
\newcommand{\gammav}{{\pmb{\gamma}}}
\newcommand{\kappav}{{\pmb{\kappa}}}
\newcommand{\muv}{{\pmb{\mu}}}
\newcommand{\omegav}{{\pmb{\omega}}}
\newcommand{\piv}{\vect{\pi}}
\newcommand{\rhov}{{\pmb{\rho}}}
\newcommand{\sigmav}{{\pmb{\sigma}}}
\newcommand{\tauv}{{\pmb{\tau}}}
\newcommand{\thetav}{{\pmb{\theta}}}
\newcommand{\xiv }{{\pmb{\xi}}}
\newcommand{\zetav}{{\pmb{\zeta}}}



\newcommand{\mat}[1]{{\pmb{#1}}} % vector in bold
\newcommand{\Am}{\mat{A}}
\newcommand{\Bm}{\mat{B}}
\newcommand{\Cm}{\mat{C}}
\newcommand{\Dm}{\mat{D}}
\newcommand{\Em}{\mat{E}}
\newcommand{\Fm}{\mat{F}}
\newcommand{\Gm}{\mat{G}}
\newcommand{\Hm}{\mat{H}}
\newcommand{\Imat}{\mat{I}}
\newcommand{\Jm}{\mat{J}}
\newcommand{\Km}{\mat{K}}
\newcommand{\Lm}{\mat{L}}
\newcommand{\Mm}{\mat{M}}
\newcommand{\Nm}{\mat{N}}
\newcommand{\Om}{\mat{O}}
\newcommand{\Pm}{\mat{P}}
\newcommand{\Qm}{\mat{Q}}
\newcommand{\Rm}{\mat{R}}
\newcommand{\Sm}{\mat{S}}
\newcommand{\Tm}{\mat{T}}
\newcommand{\Um}{\mat{U}}
\newcommand{\Vm}{\mat{V}}
\newcommand{\Wm}{\mat{W}}
\newcommand{\Xm}{\mat{X}}
\newcommand{\Ym}{\mat{Y}}
\newcommand{\Zm}{\mat{Z}}
\newcommand{\zerom}{\mat{0}}

\newcommand{\Deltam}{{\mbox{\boldmath$\Delta$}}}
\newcommand{\Gammam}{{\mbox{\boldmath$\Gamma$}}}
\newcommand{\Omegam}{{\mbox{\boldmath$\varOmega$}}}
\newcommand{\Lambdam}{{\mbox{\boldmath$\Lambda$}}}
\newcommand{\Sigmam}{{\mbox{\boldmath$\varSigma$}}}
\newcommand{\Phim}{{\mbox{\boldmath$\Phi$}}}
\newcommand{\Pim}{{\mbox{\boldmath$\Pi$}}}
\newcommand{\Thetam}{{\mbox{\boldmath$\varTheta$}}}




\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Lc}{\mathcal{L}}
\newcommand{\Kc}{\mathcal{K}}
\newcommand{\Nc}{\mathcal{N}}
\newcommand{\Xc}{\mathcal{X}}
\newcommand{\Yc}{\mathcal{Y}}
\newcommand{\Dc}{\mathcal{D}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Hc}{\mathcal{H}}
\newcommand{\Vc}{\mathcal{V}}

\newcommand{\RR}{\mathds{R}} %real numbers
\newcommand{\NN}{\mathds{N}} %natural numbers
\newcommand{\ZZ}{\mathds{Z}} %integers
\newcommand{\CC}{\mathds{C}} %complex numbers
\newcommand{\QQ}{\mathds{Q}} % rational numbers
\newcommand{\perm}{{\cal P}} %permutations
\newcommand{\transp}{\mathfrak{T}} %transpositions

\newcommand{\EE}{\mathds{E}} %expectation
\newcommand{\PP}{\mathds{P}} % proba
\newcommand{\OO}{\mathcal{O}} % grand O pour complexité
\newcommand{\ind}{\mathds{1}} % indicatrice




\DeclareMathOperator*{\diag}{\mbox{diag}}
\DeclareMathOperator*{\tr}{\mbox{tr}}
\DeclareMathOperator*{\card}{\mbox{card}}
\DeclareMathOperator*{\cov}{\mbox{cov}}
\DeclareMathOperator*{\sign}{\mbox{sign}}
\DeclareMathOperator*{\var}{\mbox{var}}
%\DeclareMathOperator*{\st}{\mbox{s.t.}}
\DeclareMathOperator*{\rank}{\mbox{rank}}

\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
%\DeclareMathOperator*{\max}{max}
%\DeclareMathOperator*{\ourargmax}{\overline{argmax}}
\DeclareMathOperator*{\ourargmax}{g-argmax}
\DeclareMathOperator*{\moyenne}{average}

\DeclareMathOperator*{\Ber}{Ber}
\DeclareMathOperator*{\Beta}{Beta}
\newcommand{\Norm}{\mathcal{N}}
\DeclareMathOperator*{\sigmoid}{sigmoid}
\DeclareMathOperator*{\logit}{logit}

\DeclareMathOperator{\KL}{kl}


\newcommand{\indep}{\perp \!\!\! \perp}
\newcommand{\defeq}{\stackrel{def}{=}}

\newcommand{\neigpermut}[3]{#1_{[#2 \Leftrightarrow #3]}}

==> supplementary_content.tex <==

The appendix is organized as follows. We first list most of the notations used in the paper in Appendix \ref{app:notations}. Lemma \ref{lem:pbm_is_unimodal} is proved in Appendix \ref{app:pbm_is_unimodal}. In Appendix \ref{app:prelim}, we recall a Lemma from \cite{Combes2014} used by our own Lemmas and Theorems, and then in Appendices \ref{app:good_leader} to \ref{app:badordering} we respectively prove Theorem \ref{theo:good_leader}, Lemma \ref{lem:bad_leader}, and Lemma \ref{lem:badordering}. In Appendix \ref{app:KL-Comb_to_PBM} we define KL-CombUCB and discuss its regret and its relation to \ouralgo{}. Finally in Appendix \ref{app:fgrab} we introduce and discuss \ouralgofull{}.



\section{Notations}\label{app:notations}

The following table summarize the notations used through the paper and the appendix.

%\begin{center}
%    \begin{small}
%        \begin{sc}
%            \begin{longtable}{ll}
%                \toprule
%                \textbf{Symbol} & \textbf{Meaning}                 \\
%                \midrule
%                \endhead
%
%                \hline \multicolumn{2}{r}{{Continued on next page}}
%                \endfoot
%
%                \bottomrule
%                \endlastfoot
%
%                \horizon        & Time horizon                     \\
%                \iteration      & Iteration                        \\
%                \nitems         & Number of items                  \\
%                \index          & index of an item                 \\
%                \intset{n}      & Set of integer $\{1,\dots , n\}$ \\
%                \carm{t}        & $\dots$                          \\
%                \leader{t}      & $\dots$                          \\
%                \optimum        & $\dots$                          \\
%            \end{longtable}
%        \end{sc}
%    \end{small}
%\end{center}

\begin{center}
\begin{small}
\begin{sc}
    \begin{longtable}{ll}
        \toprule
        \textbf{Symbol} &\textbf{Meaning}\\
        \midrule
        \endhead
        
        \hline \multicolumn{2}{r}{{Continued on next page}}
        \endfoot
        
        \bottomrule
        \endlastfoot

         T& Time horizon\\
        $t$& iteration \\
        L& number of items \\
        $i$& index of an item \\
        K& number of positions in a recommendation\\
        $k$ & index of a position \\
        $[n]$ & set of integers $\{1,\dots,n\}$\\
        $\perm_K^L$ & set of permutations of K distinct items among L\\
        $\thetav$& vectors of probabilities of click\\
        $\theta_i$& probability of click on item $i$ \\
        $\kappav$& vectors of probabilities of view \\
        $\kappa_k$& probability of view at position $k$ \\
        $\Ac$ & set of bandit arms\\
        $\av$ & an arm in  $\Ac$ \\
        $\av(t)$ & the arm chosen at iteration $t$ \\
        $\tilde \av(t)$ & best arm at iteration $t$ given the previous choices and feedbacks (called leader)  \\
        $\av^*$ & best arm \\
        $G$ & graph carrying a partial order on $\Ac$ \\
        $\gamma$ & maximum degree of $G$ \\
        $\Nc_G(\tilde \av(t))$ & neighborhood of $\tilde a(t)$ given $G$ \\
        $\rho_{i,k}$& probability of click on item $i$ displayed at position $k$ \\
        $\cv(t)$& clicks vector at iteration $t$ \\
        $r(t)$ & reward collected at iteration $t$, $r(t)=\sum_{k=1}^K c_k(t)$\\
        $\mu_\av$& expectation of $r(t)$ while recommending $\av$, $\mu_\av=\sum_{k=1}^K \rho_{a_k,k}$ \\
        $\mu^*$& highest expected reward, $\mu^*=\max_{\av\in \perm_K^L}\mu_\av$\\
        $\Delta_a$& gap between $\mu_a$ and $\mu^*$ \\
        $\Delta_{min}$& minimal value for $\Delta_a$\\ 
        $\Delta$& generic reward gap between one of the sub-optimal arms and one of the best arms\\
        $R(T)$ & cumulative (pseudo-)regret, $R(T) = T\mu^* - \EE\left[\sum_{t = 1}^T \mu_{\av(t)}\right]$\\
        $\Pi_\rhov(\av)$& set of permutations in $\perm_K^K$ ordering the positions s.t. $\rho_{a_{\pi_{1}},\pi_{1}} \geqslant \rho_{a_{\pi_{2}},\pi_{2}} \geqslant \dots \geqslant \rho_{a_{\pi_{K}},\pi_{K}}$\\
        $\piv$& element of  $\Pi_\rhov(\av)$\\
        $\tilde\piv$& estimation of $\piv$\\
        $\av \circ (\pi_{k}, \pi_{k+1})$ & permutation swapping items in positions $\pi_{k}$ and $\pi_{k+1}$\\
        $\av[\pi_{K} := i]$& permutation leaving $\av$ the same for any position except $\pi_{K}$ for which $\av[\pi_{K}~:=~i]_{\pi_{K}}=i$\\
        ${\mapping}$ & rankings of positions respecting $\Pi_\rhov$,  ${\mapping} =\left(\piv_\av\right)_{\av \in \perm_K^L}$ s.t. $\forall \av\in \perm_K^L, \piv_\av\in\Pi_\rhov(\av)$\\
        $T_{i,k}(t)$ & number of iterations s.t. item $i$ has been displayed at position $k$, $T_{i,k}(t) = \sum_{s = 1}^{t-1} \ind\{a_k(s) = i\}$\\
        $\tilde{T}_\av(t)$ &  number of iterations s.t. the leader was $\av$, $\tilde{T}_\av(t) \defeq \sum_{s = 1}^{t-1} \ind\{\tilde\av(s) = \av\}$ \\
        $T_\av(t)$ &  number of iterations s.t. the chosen arm was $\av$, $T_\av(t) = \sum_{s = 1}^{t-1} \ind\{\av(s) = \av\}$ \\
        $T_\av^{\tilde\av}(t)$ & number of iterations s.t. the leader was $\tilde\av$, the chosen arm was $\av$, and $\av$ was chosen
        \\& by the argmax on $\sum_{k=1}^K b_{a_k, k}(t)$: $T_{\av}^{\tilde\av}(t) = \sum_{s=1}^{t-1} \ind\left\{\tilde\av(s)=\tilde\av, \av(s) = \av, \tilde{T}_{\tilde\av}(s)/L \notin \NN\right\}$\\
        $\hat\rho_{i,k}(t)$& estimation of $\rho_{i,k}$ at iteration $t$,  $\hat\rho_{i,k}(t) = \frac{1}{T_{i,k}(t)}\sum_{s = 1}^{t-1} \ind\{a_k(s) = i\}c_k(s)$\\
        $b_{i,k}(t)$ & Kullback-Leibler index of $\hat\rho_{i,k}(t)$ , $b_{i,k}(t) = f\left(\hat\rho_{i,k}(t), T_{i,k}(t), \tilde{T}_{\tilde\av(t)}(t)+1\right)$ \\
        $f$ & Kullback-Leibler index function, $f(\hat\rho, s, t) = \sup \{p\in[\hat\rho,1]: s\times\KL(\hat{\rho}, p) \leq \log (t) + 3 \log(\log (t))\},$\\
        $\KL(p,q)$ & Kullback-Leibler divergence from a Bernoulli distribution of mean $p$\\
        &to a Bernoulli distribution of mean $q$,  $\KL(p,q) = p \log \left(\frac{p}{q}\right) + (1-p)\log \left(\frac{1 - p}{1 - q}\right)$ \\
        $B_{\av}(t)$ & pseudo-sum of indices of $\av$ at iteration t, $B_{\av}(t) = \sum_{k=1}^K b_{a_k, k}(t) - \sum_{k=1}^K b_{\tilde{a}_k(t), k}(t)$\\
        $\Nc_{\pi^*}(a^*)$& neighborhood of the best arm\\
%        $P^L_K$& number of K-permutations of L items\\
%        $P_{max}$& size of the larger set of $\Pi_\rhov(\av)$\\
        $K_\av$& (with combinatorial bandit setting) number of elements in $\av$ but not in $\av^*$,\\& $K_\av = \min_{\av^*\in\Ac: \mu_{\av^*}=\mu^*} |\av\setminus\av^*|$\\
        $K_{max}$& (with combinatorial bandit setting) maximal number of elements in a sub-optimal arm $\av$\\& but not in an optimal arm $a^*$, $K_{max}=\max_{\av \in\Ac: \mu_\av\neq\mu^*} K_\av$\\
        $c^*\left(\thetav, \kappav\right)$ & coefficient in the regret bound of PMED\\
        $c$ & (in $\varepsilon_n$-greedy) parameter controlling the probability of exploration\\
        $c$ & (in PB-MHB) parameter controlling size of the step in the Metropolis Hasting inference \\
        $m$ & (in PB-MHB) number of step in the Metropolis Hasting inference \\
\end{longtable}
\end{sc}
\end{small}
\end{center}


\section{Proof of Lemma \ref{lem:pbm_is_unimodal} (PBM Fulfills Assumption 1) }\label{app:pbm_is_unimodal}

\begin{proof}[Proof of Lemma \ref{lem:pbm_is_unimodal}]
Let $(L, K, (\rho_{i,k})_{(i,k)\in [L]\times[K]})$ be an online learning to rank (OLR) problem with users following PBM, with positive probabilities of looking at a given position. Therefore, there exists $\thetav\in[0,1]^L$ and $\kappav\in(0,1]^K$ such that for any item $i$ and any position $k$, $\rho_{i,k}=\theta_i\kappa_k$.

Let $\av\in\perm_K^L$ be a recommendation, and let $\piv\in \Pi_\rhov\left(\av\right)$ be an appropriate ranking of positions. One of the four following properties is satisfied:
\begin{align}
    &\exists k \in [K-1]\text{ s.t. } \theta_{a_{\pi_k}} < \theta_{a_{\pi_{k+1}}}, \label{eq:thetabadinside}\\
    &\exists k \in [K-1]\text{ s.t. } \kappa_{\pi_k} < \kappa_{\pi_{k+1}},\label{eq:kappabad}\\
    &\exists i \in [L]\setminus\av([K])\text{ s.t. } \theta_{a_{\pi_K}} < \theta_{i},\label{eq:thetabadoutside}\\
    &\begin{cases}
        \forall k \in [K-1], \theta_{a_{\pi_k}} \geqslant  \theta_{a_{\pi_{k+1}}}\\
        \forall k \in [K-1], \kappa_{\pi_k} \geqslant \kappa_{\pi_{k+1}}\\
        \forall i \in [L]\setminus\av([K]), \theta_{a_{\pi_K}} \geqslant \theta_{i}
    \end{cases}\label{eq:everythingok}.
\end{align}

Let prove, by considering each of these properties one by one, that $\av$ is either one of the best arms, or $\av$ fulfills either Property (2) or Property (3) of Assumption 1.

If Property \eqref{eq:thetabadinside} is satisfied and $\theta_{a_{\pi_k}}=0$, then by definition of $\piv$ and $\Pi_\rhov\left(\av\right)$, $0=\theta_{a_{\pi_k}}\kappa_{\pi_k} \geqslant \theta_{a_{\pi_{k+1}}}\kappa_{\pi_{k+1}} >0$ which is absurd. 

Therefore, If Property \eqref{eq:thetabadinside} is satisfied, $\frac{\theta_{a_{\pi_{k+1}}}}{\theta_{a_{\pi_k}}} > 1.$

Note that by definition of $\piv$ and $\Pi_\rhov\left(\av\right)$, and as $\rho_{i,k}=\theta_i\kappa_k$,
$\theta_{a_{\pi_k}}\kappa_{\pi_k} \geqslant \theta_{a_{\pi_{k+1}}}\kappa_{\pi_{k+1}}$.

Hence $\kappa_{\pi_k} \geqslant \frac{\theta_{a_{\pi_{k+1}}}}{\theta_{a_{\pi_k}}} \kappa_{\pi_{k+1}} > \kappa_{\pi_{k+1}}$,
and
\begin{align*}
    \mu_\av - \mu_{\av\circ\left(\pi_k, \pi_{k+1}\right)}
    &=  \theta_{a_{\pi_k}}\kappa_{\pi_k} + \theta_{a_{\pi_{k+1}}}\kappa_{\pi_{k+1}}
    - \left(\theta_{a_{\pi_{k+1}}}\kappa_{\pi_k} + \theta_{a_{\pi_k}}\kappa_{\pi_{k+1}}\right)
    \\
    &= \left(\theta_{a_{\pi_k}} - \theta_{a_{\pi_{k+1}}}\right)
    \left(\kappa_{\pi_k} - \kappa_{\pi_{k+1}}\right)
    \\
    &< 0,
\end{align*}
meaning $\mu_\av < \mu_{\av\circ\left(\pi_k, \pi_{k+1}\right)}$, which corresponds to Property (2) of Assumption 1.

Similarly, if Property \eqref{eq:kappabad} is satisfied, then
Property (2) of Assumption 1 is fulfilled.

If Property \eqref{eq:thetabadoutside} is satisfied,
\begin{align*}
    \mu_\av - \mu_{\av[\pi_{K} := i]}
    &=  \theta_{a_{\pi_K}}\kappa_{\pi_K} - \theta_{i}\kappa_{\pi_K}
    \\
    &= \left(\theta_{a_{\pi_K}} - \theta_{i}\right)\kappa_{\pi_K}
    \\
    &< 0.
\end{align*}
Hence $\mu_\av < \mu_{\av[\pi_{K} := i]}$, which corresponds to Property (3) of Assumption 1.

Finally, if Property \eqref{eq:everythingok} is satisfied, $\mu_\av = \mu^*$.

Overall, either $\av$ is one of the best arms, or $\av$ fulfills Property (2) of Assumption 1, or $\av$ fulfills Property (3) of Assumption 1, which concludes the proof.


\end{proof}




\section{Preliminary to the Analysis of \ouralgo{}}\label{app:prelim}

The analysis of \ouralgo{} requires a control of the number of high deviations, as expressed by Lemma $B.1$ of \cite{Combes2014}. Let us recall this lemma, which we denote Lemma \ref{lem:B1} in current paper. 

\begin{lemma}[Lemma B.1 of \cite{Combes2014}]\label{lem:B1}
Let $i\in [L]$, $k\in[K]$, $\epsilon>0$.
Define $\Fc(T)$ the $\sigma$-algebra generated by $\left(\cv(t)\right)_{t\in [T]}$.
Let $\Lambda\subseteq\NN$ be a random set of instants. Assume that there exists a sequence of random sets $\left(\Lambda(s)\right)_{s\geq1}$ such that (i)  $\Lambda\subseteq\bigcup_{s\geq1}\Lambda(s)$, (ii) for all $s\geqslant 1$ and all $t\in \Lambda(s)$, $T_{i,k}(t)\geq\epsilon s$, (iii) $|\Lambda(s)|\leqslant 1$, and (iv) the event $t\in \Lambda(s)$ is $\Fc_t$-measurable. Then for all $\delta>0$,

$$\EE\left[\sum_{t\geq1} \ind\{t \in \Lambda,  |\hat\rho_{i, k}(t) - \rho_{i, k}| \geqslant \delta \}\right]\\
 \leqslant \frac{1}{\epsilon\delta^2}$$
\end{lemma}


\section{Proof of Theorem \ref{theo:good_leader} (Upper-bound on the Regret of  KL-CombUCB)}\label{app:good_leader}



\begin{proof}[Proof of Theorem \ref{theo:good_leader}]
Let $\av\in \Ac$ be a sub-optimal arm. 
Let $\av^*\in \Ac$ be an optimal arm such that $|\av\setminus\av^*| = K_\av$.

We denote $\bar{K}_\av\defeq |\av^*\setminus\av|$,
$T_\av(t) \defeq \sum_{s = 1}^{t-1} \ind\{\av(s) = \av\}$
the number of time the arm $\av$ has been drawn,
and $T_e(t) \defeq \sum_{s = 1}^{t-1} \ind\{e \in \av(s)\}$ the number of time the element $e$ was in the drawn arm. 

Let decompose the expected number of iterations at which the permutation $\av$ is recommended:
\begin{align*}
\EE\left[\sum_{t=1}^T \ind\{\av(t) = \av\}\right]
    &\leqslant \sum_{e \in \av\setminus\av^*}\EE\left[\sum_{t=1}^T \ind\left\{\av(t) = \av, |\hat\rho_e(t) - \rho_e|\geqslant \frac{\Delta_\av}{2K_\av}  \right\}\right]
\\
    &\quad + \sum_{e \in \av^*\setminus\av}\EE\left[\sum_{t=1}^T \ind\{b_e(t) \leqslant \rho_e \}\right]
    \\
    &\quad +  \EE\left[\sum_{t=|E|}^{T} \ind\left\{\av(t) = \av, \forall e \in \av\setminus\av^*, |\hat\rho_e(t) - \rho_e|< \frac{\Delta_\av}{2K_\av},  \forall e \in \av^*\setminus\av, b_e(t) > \rho_e \right\}\right]
    \\
    &\quad + |E|
    .
\end{align*}
The proof consists in upper-bounding each term on the right-hand side.


\paragraph{First Term}
Let $e \in \av\setminus\av^*$, and denote $A_e = \left\{t\in [T]: \av(t) = \av, |\hat\rho_e(t) - \rho_e|\geqslant \frac{\Delta_\av}{2K_\av}\right\}$.

$A_e \subseteq \bigcup_{s\in \NN} \Lambda_k(s)$, where $\Lambda_k(s) \defeq \{t\in A_e : T_{\av}(t)=s\}$. For any integer value $s$, $|\Lambda_k(s)| \leqslant 1$ as  $T_\av(t)$ increases for each $t\in A_e$. Note that for each $s\in \NN$ and $n\in \Lambda_k(s)$, $T_e(n) \geqslant T_\av(n)=s$. Then, by Lemma \ref{lem:B1}

\begin{align*}
    \EE\left[|A_e|\right]
    &\leq\EE\left[\sum_{t=1}^T \ind\{t \in A_e\}\right]\\
    & = \EE\left[\sum_{t=1}^T \ind\left\{t \in A_e,  |\hat\rho_e(t) - \rho_e| \geqslant \frac{\Delta_\av}{2K_\av} \right\}\right]\\
    & \leqslant \frac{4K_\av^2}{\Delta_\av^2}.
\end{align*}
Hence, $ \sum_{e \in \av\setminus\av^*}\EE\left[\sum_{t=1}^T \ind\left\{\av(t) = \av, |\hat\rho_e(t) - \rho_e|\geqslant \frac{\Delta_\av}{2K_\av}  \right\}\right]
= \sum_{e \in \av\setminus\av^*} \EE\left[|A_e|\right]
\leqslant \frac{4K_\av^3}{\Delta_\av^2}$.

\paragraph{Second Term}
Let $e \in \av^*\setminus\av$, and denote $B_e \defeq \{t\in [T]: b_e(t) \leqslant \rho_e\}$.

By Theorem 10 of \cite{Garivier2011}, $\EE\left[|B_e|\right] = O(\log\log T)$, so $ \sum_{e \in \av^*\setminus\av}\EE\left[\sum_{t=1}^T \ind\{b_e(t) \leqslant \rho_e \}\right] = \OO(\bar{K}_\av\log \log T)$.

\paragraph{Third Term}
Let note $C \defeq \left\{t\in [T]\setminus[|E|]: \av(t) = \av, \forall e \in \av\setminus\av^*, |\hat\rho_e(t) - \rho_e|< \frac{\Delta_\av}{2K_\av},  \forall e \in \av^*\setminus\av, b_e(t) > \rho_e\right\}$.

Let $t\in C$.

At each step of the initialization phase, the algorithm removes at least one element $e$ of the set $\tilde{E}$ of unseen elements. Therefore, the initialization lasts at most $|E|$ iterations. Hence, at iteration $t$, $\av(t)=\av$ is chosen as $\sum_{e\in\av} b_e(t) = \max_{\av'\in\Ac}\sum_{e\in\av'} b_e(t)$.

Then, by Pinsker's inequality and the fact that $t\leqslant T$, and $T_e(t) \geqslant T_\av(t)$ for any $e$ in $\av$,
\begin{align*}
    0
    & \leqslant \sum_{e\in\av} b_e(t) - \sum_{e\in\av^*}  b_e(t)
    \\
    &= \sum_{e\in\av\setminus\av^*} b_e(t) - \sum_{e\in\av^*\setminus\av}  b_e(t)
    \\
    &\leqslant \sum_{e\in\av\setminus\av^*} \hat\rho_e(t) +  \sqrt{\frac{\log(t)+3\log(\log(t))}{2T_e(t)}}
    - \sum_{e\in\av^*\setminus\av} b_e(t)
    \\
    &< \sum_{e\in\av\setminus\av^*} \rho_e + \frac{\Delta_\av}{2K_\av} + \sqrt{\frac{\log(T)+3\log(\log(T))}{2 T_\av(t)}}
    - \sum_{e\in\av^*\setminus\av} \rho_e
    \\
    &\leqslant \sum_{e\in\av} \rho_e - \sum_{e\in\av^*} \rho_e 
    + K_\av \frac{\Delta_\av}{2K_\av}
    + K_\av\sqrt{\frac{\log(T)+3\log(\log(T))}{2 T_\av(t)}} 
    \\
    &= -\Delta_\av  + \frac{2\Delta_\av}{2} +  K_\av\sqrt{\frac{\log(T)+3\log(\log(T))}{2 T_\av(t)}}.
    \\
    &= - \frac{\Delta_\av}{2} +  K_\av\sqrt{\frac{\log(T)+3\log(\log(T))}{2 T_\av(t)}}.
\end{align*}

Hence, $T_\av(t) <  K_\av^2\frac{2\log(T)+6\log(\log(T))}{\Delta_\av^2}$.
Therefore, $C\subseteq \left\{t\in [T]\setminus[|E|]: \av(t) = \av, T_\av(t) < K_\av^2\frac{2\log(T)+6\log(\log(T))}{\Delta_\av^2}\right\}$, and

\begin{align*}
    \EE&\left[\sum_{t=|E|}^{T} \ind\left\{\av(t) = \av, \forall e \in \av\setminus\av^*, |\hat\rho_e(t) - \rho_e|< \frac{\Delta_\av}{2K_\av},  \forall e \in \av^*\setminus\av, b_e(t) > \rho_e \right\}\right]
    \\
    &= \EE\left[|C|\right]
    \\
    &\leqslant \EE\left[\left|\left\{t\in [T]\setminus[|E|]: \av(t) = \av, T_\av(t) < K_\av^2\frac{2\log(T)+6\log(\log(T))}{\Delta_\av^2}\right\}\right|\right]
    \\
    &\leqslant K_\av^2\frac{2\log(T)+6\log(\log(T))}{\Delta_\av^2}.
\end{align*}

\paragraph{Regret upper-bound}
Overall,
\begin{align*}
\EE\left[\sum_{t=1}^T \ind\{\av(t) = \av\}\right]
&\leqslant \frac{4K_\av^3}{\Delta_\av^2}
+ \OO(\bar{K}_\av\log \log T)
+ K_\av^2\frac{2\log(T)+6\log(\log(T))}{\Delta_\av^2}
+ |E|
\\
& = \frac{2K_\av^2}{\Delta_\av^2}\log(T)
+ \OO\left(\left(\bar{K}_\av+\frac{K_\av^2}{\Delta_\av^2}\right)\log \log T\right)
\end{align*}
%
and
%
\begin{align*}
R(T)
&=\sum_{\av \in \Ac : \mu_\av \neq \mu^*} \Delta_\av \EE\left[\sum_{t=1}^T \ind\{\av(t) = \av\}\right]
\\
&\leqslant \sum_{\av \in \Ac : \mu_\av \neq \mu^*} \frac{2K_\av^2}{\Delta_\av}\log(T)
+ \OO\left(\left(\bar{K}_\av\Delta_\av+\frac{K_\av^2}{\Delta_\av}\right)\log \log T\right)
\\
&=\OO\left(\frac{|\Ac|K_{max}^2}{\Delta_{\text{min}}}\log T\right),
\end{align*}
which concludes the proof.

\end{proof}


\section{Proof of Lemma \ref{lem:bad_leader} (Upper-bound on the Number of Iterations of \ouralgo{} for which $\tilde\av(t)=\tilde\av\neq\av^*$)}\label{app:bad_leader}

\begin{proof}[Proof of Lemma \ref{lem:bad_leader}]
Let $\tilde\av \in\perm_K^L\setminus\{\av^*\}$ and prove that $\EE\left[\sum_{t=1}^T\ind\{\tilde\av(t)=\tilde\av\}\right]
= \OO\left(\log\log T\right)$.
%As for any ranking of positions $\tilde\piv \in \Pi_\rhov\left(\tilde\av\right)$, $\EE\left[\sum_{t=1}^T\ind\{\tilde\av(t)=\tilde\av, \tilde\piv(t)=\tilde\piv\}\right]\leqslant\EE\left[\sum_{t=1}^T\ind\{\tilde\av(t)=\tilde\av\}\right]$, it will prove Lemma \ref{lem:bad_leader}.

The proof requires notations related to the neighborhood of $\tilde\av$. Let $\Nc \defeq \bigcup_{\piv\in\perm_K^K}\Nc_\piv(\tilde\av)$
be the set of all the potential neighbors of $\tilde\av$. By definition of the neighborhoods,
$$\Nc=\left\{\tilde\av \circ (k,k'):  k,k' \in [K]^2, k>k'\right\} \cup
\left\{\tilde\av[k := i]: k \in [K], i \in [L]\setminus\tilde\av([K])\right\},$$
and its size is $N=K(2L-K-1)/2$.
As $\tilde\av$ is sub-optimal, and due to Assumption 1, for any appropriate ranking of positions $\piv \in \Pi_\rhov\left(\tilde\av\right)$, there exists a recommendation $\av^+$ with a strictly better expected reward than $\tilde\av$ in the neighborhood $\Nc_\piv(\tilde\av)$. We denote
$$\Nc^+\defeq\bigcup_{\piv \in \Pi_\rhov\left(\tilde\av\right)} \left\{\av^+\in\Nc_\piv(\tilde\av) : \mu_{\av^+} = \max_{\av\in\Nc_\piv(\tilde\av)}\mu_\av\right\}$$
the set of such recommendations. We also chose $\epsilon<\min\{1/(2N), 1/L\}$ and note
$$\delta \defeq \min_{\piv \in \Pi_\rhov\left(\tilde\av\right)}
\min_{\av \in \Nc_{\piv}(\tilde\av) \cup \{\tilde\av\}\setminus\Nc^+}
\left(\max_{\av'\in\Nc_\piv(\tilde\av)}\mu_{\av'} - \mu_\av\right).$$


To bound $\EE\left[\ind\{\tilde\av(t)=\tilde\av\}\right]$, we use the decomposition
$\{t \in [T]: \tilde\av(t)=\tilde\av\} \subseteq \bigcup_{\av^+\in \Nc^+} A_{\av^+} \cup B$ where for any permutation $\av^+\in\Nc^+$,
$$A_{\av^+} = \{t : \tilde\av(t)=\tilde\av, T_{\av^+}(t) \geqslant \epsilon \tilde{T}_{\tilde\av}(t) \}$$
and
$$B = \{t : \tilde\av(t)=\tilde\av, \forall \av^+ \in \Ac+, T_{\av^+}(t) < \epsilon \tilde{T}_{\tilde\av}(t) \}.$$
Hence, 
$$\EE\left[\ind\{\tilde\av(t)=\tilde\av\}\right]
\leqslant \sum_{\av^+ \in \Ac+} \EE\left[|A_{\av^+}|\right]
+ \EE\left[|B|\right].$$

\paragraph{Bound on $\EE\left[|A_{\av^+}|\right]$}
Let $\av^+$ be a permutation in $\Nc^+$ and denote $\Kc^+$ the set of positions for which  $\av^+$ and $\tilde\av$ disagree: $\Kc^+=\left\{k\in[K] : a^+_k \neq \tilde{a}_k\right\}$.
The permutation $\av^+$ is in the neighborhood of $\tilde\av$, so either ${\av^+} = \tilde\av \circ (k, k')$ or ${\av^+} = \av[k := i]$, with $k$ and $k'$ in $[K]$, and $ i$ in $[L]$. Overall, $|\Kc^+| \leqslant 2$.

By the design of the algorithm and by definition of $\epsilon$, we have that $\forall t \in A_{\av^+}$, $T_{\tilde\av}(t) \geqslant \tilde{T}_{\tilde\av}(t)/L > \epsilon \tilde{T}_{\tilde\av}(t)$.
Moreover, at the considered iterations $\tilde\av$ is the leader, so 
\begin{align*}
A_{\av^+} &
  \subseteq \left\{t: \tilde\av(t)=\tilde\av, \tilde{T}_{\tilde\av}(t)<\frac{1}{\epsilon} \right\}
  \cup\left\{t: \tilde\av(t)=\tilde\av, \min\{T_{\tilde\av}(t), T_{\av^+}(t)\} \geqslant \epsilon \tilde{T}_{\tilde\av}(t)\geqslant 1, \muh{\tilde{a}} \geqslant \muh{a^+} \right\}
\\
  &\subseteq \left\{t: \tilde\av(t)=\tilde\av, \tilde{T}_{\tilde\av}(t)<\frac{1}{\epsilon} \right\}
  \cup \left\{t: \tilde\av(t)=\tilde\av, \min\{T_{\tilde\av}(t), T_{\av^+}(t)\} \geqslant \epsilon \tilde{T}_{\tilde\av}(t),  \sum_{k\in\Kc^+}\hat\rho_{\tilde{a}_k,k}(t)
\geqslant \sum_{k\in\Kc^+}\hat\rho_{a^+_k,k}(t) \right\}
\\
 &\subseteq \left\{t: \tilde\av(t)=\tilde\av, \tilde{T}_{\tilde\av}(t)<\frac{1}{\epsilon} \right\}
  \\&\quad\cup \left\{t: \tilde\av(t)=\tilde\av, \min\{T_{\tilde\av}(t), T_{\av^+}(t)\} \geqslant \epsilon \tilde{T}_{\tilde\av}(t),
\exists k\in \Kc^+,
 |\hat\rho_{\tilde{a}_{k}, k}(t) - \rho_{\tilde{a}_{k}, k}| \geqslant \frac{\delta}{2|\Kc^+|}
 \text{ or } 
 |\hat\rho_{a^+_{k}, k}(t) - \rho_{a^+_{k}, k}| \geqslant \frac{\delta}{2|\Kc^+|}
\right\}
\\
 &\subseteq \left\{t: \tilde\av(t)=\tilde\av, \tilde{T}_{\tilde\av}(t)<\frac{1}{\epsilon} \right\}
  \cup \bigcup_{k\in\Kc^+}\bigcup_{i\in\left\{\tilde{a}_k, a^+_k\right\}}
 \Lambda_{i, k},
\end{align*}
with $\Lambda_{i, k} \defeq \left\{t: \tilde\av(t)=\tilde\av, \min\{T_{\tilde\av}(t), T_{\av^+}(t)\} \geqslant \epsilon \tilde{T}_{\tilde\av}(t),
 |\hat\rho_{i, k}(t) - \rho_{i, k}| \geqslant \frac{\delta}{2|\Kc^+|}
\right\}$.

Fix $k$ in $\Kc^+$ and $i$ in $\left\{\tilde{a}_k, a^+_k\right\}$.
$\Lambda_{i,k} \subseteq \bigcup_{s\in\NN}\Lambda_{i,k}(s)$, with $\Lambda_{i,k}(s) \defeq \{t\in \Lambda_{i,k}: \tilde{T}_{\tilde\av}(t) = s\}$. $|\Lambda_{i,k}(s)| \leqslant 1$ as $\tilde{T}_{\tilde\av}(t)$ increases for each $t\in \Lambda_{i,k}$.  Note that for each $s\in \NN$ and $n \in \Lambda_{i,k}(s)$, $T_{i,k}(n) \geqslant \min\left\{T_\av(n), T_{\av^+}(n)\right\} \geqslant \epsilon\tilde{T}_{\tilde\av}(n)=\epsilon s$. Then, by Lemma \ref{lem:B1}
\begin{align*}
\EE\left[|\Lambda_{i,k}|\right]
&=\EE\left[\sum_{t=1}^T \ind\{t \in \Lambda_{i,k}\}\right]\\
& = \EE\left[\sum_{t=1}^T \ind\left\{t \in \Lambda_{i,k}, |\hat\rho_{i,k}(t) - \rho_{i,k}| > \frac{\delta}{2|\Kc^+|} \right\}\right]\\
& \leqslant \frac{4|\Kc^+|^2}{\epsilon\delta^2}
\end{align*}
Hence, $\EE\left[|A_{\av^+}|\right] \leqslant \frac{1}{\epsilon} + \sum_{k\in\Kc^+}\sum_{i\in\left\{\tilde{a}_k, a^+_k\right\}} \EE\left[|\Lambda_{i, k}|\right]  \leqslant \frac{1}{\epsilon} + \frac{8|\Kc^+|^3}{\epsilon\delta^2}$.

\paragraph{Bound on $\EE\left[|B|\right]$}
We first split $B$ in two parts: $B=B^{t_0} \cup B_{t_0}^T$, where $B^{t_0}\defeq \{t\in B: \tilde{T}_{\tilde\av}(t)\leqslant t_0\}$, $B_{t_0}^T\defeq \{t\in B: \tilde{T}_{\tilde\av}(t) > t_0\}$, and $t_0$ is chosen as small as possible to satisfy three constraints required in the rest of the proof.

Namely, $t_0 = \max \left\{
\frac{1}{\epsilon},
(1+N)(1-\frac{1}{L}-\epsilon N)^{-1},
\inf \left\{t: 2\sqrt{\frac{\log (t+1) + 3\log(\log (t+1))}{2\epsilon t}} < \frac{\delta}{8}\right\} \right\}$. Note that $t_0$ only depends on $K$, $L$  and $\delta$, and that $(1-\frac{1}{L}-\epsilon N) > 0$ (assuming $L \geqslant 2$) as $\epsilon < 1/(2N)$.

We also define
\begin{itemize}
    \item $D \defeq \bigcup_{(\av,k) \in (\Nc\cup\{\tilde\av\}\setminus\Nc^+)\times[K]}D_{\av,k}$, where
    $D_{\av,k} \defeq \left\{t \in [T]:  \tilde\av(t)=\tilde\av, \av(t)=\av
    , |\hat\rho_{a_k, k}(t) - \rho_{a_k, k}| \geqslant \frac{\delta}{8}\right\},$
    \item $E \defeq \bigcup_{(\av^+,k)\in \Nc^+\times [K]}E_{\av^+,k}$, where
    $E_{\av^+,k} \defeq \{t \in [T]:  \tilde\av(t)=\tilde\av, b_{a^+_{k},k}(t) \leqslant \rho_{a^+_{k},k} \},$
    \item and $F \defeq\{t \in [T]: \tilde\av(t)=\tilde\av, \tilde\piv(t)\notin\Pi_\rhov\left(\tilde\av\right)\}.$
\end{itemize}



Let $t \in B_{t_0}^T$. By construction, \ouralgo{} forces itself to select $\left\lceil \frac{\tilde{T}_{\tilde\av}(t)}{L} \right\rceil$ times the leader $\tilde\av$  between iterations 1 and $t-1$. So, 
$$\tilde{T}_{\tilde\av}(t)  = \left\lceil \frac{\tilde{T}_{\tilde\av}(t)}{L} \right\rceil + \sum_{\av \in \Nc\cup\{\tilde\av\}}T_{\av}^{\tilde\av}(t)$$
where $T_{\av}^{\tilde\av}(t) = \sum_{s=1}^{t-1} \ind\left\{\tilde\av(s)=\tilde\av, \av(s) = \av, \tilde{T}_{\tilde\av}(s)/L \notin \NN\right\}$ is the number of times arm $\av \in \Nc\cup\{\tilde\av\}$ has been played \textbf{normally} (i.e not forced) while $\tilde\av$ was leader, up to time $t-1$. Let prove by contradiction that there is at least one recommendation $\av$ that has been selected \textbf{normally} more than $\epsilon \tilde{T}_{\tilde\av}(t)+1$ times, namely $T_{\av}^{\tilde\av}(t)\geqslant \epsilon \tilde{T}_{\tilde\av}(t)+1$.

Assume that for each recommendation $\av$ in $\Nc\cup\{\tilde\av\}$, $T_{\av}^{\tilde\av}(t) < \epsilon \tilde{T}_{\tilde\av}(t)+1$. Then
\begin{align*}
\tilde{T}_{\tilde\av}(t)
&= \left\lceil \frac{\tilde{T}_{\tilde\av}(t)}{L} \right\rceil + \sum_{\av \in \Nc\cup\{\tilde\av\}}T_{\av}^{\tilde\av}(t)\\
&< 1 + \frac{\tilde{T}_{\tilde\av}(t)}{L}
+ N (\epsilon \tilde{T}_{\tilde\av}(t) +1).
\end{align*}
Therefore
$\tilde{T}_{\tilde\av}(t) (1- \frac{1}{L} - N \epsilon ) < 1 + N$, which contradicts $t\in B_{t_0}^T$. 


So, there exists a  recommendation $\av$ such that $T_{\av}^{\tilde\av}(t)\geqslant \epsilon \tilde{T}_{\tilde\av}(t)+1$. Let denote $s'$ the first iteration such that $T_{\av}^{\tilde\av}(s')\geqslant \epsilon \tilde{T}_{\tilde\av}(t)+1$. At this iteration,  $T_{\av}^{\tilde\av}(s') =T_{\av}^{\tilde\av}(s'-1) +1$, meaning that $\tilde\av(s'-1) = \tilde\av$,  $\av(s'-1)=\av$,  $\tilde{T}_{\tilde\av}(s'-1)/L \notin \NN$, and $T_{\av}^{\tilde\av}(s'-1)\geqslant \epsilon \tilde{T}_{\tilde\av}(t)$. Therefore, the set  $\{s \in [t]: \tilde\av(s) = \tilde\av, T_{\av(s)}^{\tilde\av}(s) \geqslant \epsilon \tilde{T}_{\tilde\av}(t),   \tilde{T}_{\tilde\av}(s)/L \notin \NN \}$ is non-empty. We define $\psi(t)$ as the minimum on this set
$$ \psi(t) \defeq \min\left\{s \in [t]: \tilde\av(s) = \tilde\av, T_{\av(s)}^{\tilde\av}(s) \geqslant \epsilon \tilde{T}_{\tilde\av}(t),   \tilde{T}_{\tilde\av}(s)/L \notin \NN \right\}.$$


We note $\av$ the recommendation $\av(\psi(t))$ at iteration $\psi(t)$.
We have $\av \notin \Nc^+$ since for any recommendation $\av^+ \in\Nc^+$, $T_{\av^+}^{\tilde\av}(\psi(t)) \leqslant T_{\av^+}^{\tilde\av}(t) \leqslant T_{\av^+}(t) < \epsilon \tilde{T}_{\tilde\av}(t)$.
Let $\av^+$ be one of the best recommendations in $\Nc_{\tilde\piv\left(\psi(t)\right)}\left(\tilde\av\right)\cup\{\tilde\av\}$, meaning $\mu_{\av^+} = \max_{\av'\in \Nc_{\tilde\piv\left(\psi(t)\right)}\left(\tilde\av\right)\cup\{\tilde\av\}}\mu_{\av'}$,
and let $\Kc$ denote the set of positions for which $\av$ and $\av^+$ disagree. As both recommendations are in  $\Nc_{\tilde\piv\left(\psi(t)\right)}(\tilde\av)\cup\{\tilde\av\}$, $|\Kc|\leqslant 4$.


Let prove by contradiction that $\psi(t) \in D \cup E \cup F$. Assume that $\psi(t) \notin D \cup E \cup F$. 

Since $\psi(t) \notin F$, $\tilde\piv\left(\psi(t)\right)$ belongs to $\Pi_\rhov\left(\tilde\av\right)$ and hence $\av{^+}$ is in $\Nc^+$ and $\sum_k \rho_{a^+_k, k} - \sum_k \rho_{a_k, k} =\mu_{\av^+}-\mu_\av\geqslant \delta$.


Moreover, since $\psi(t) \notin D \cup E$, for each position $k\in[K]$, $ |\hat\rho_{a_k, k}(\psi(t)) - \rho_{a_k, k}| < \frac{\delta}{8}$, and $b_{a^+_{k},k}(\psi(t)) > \rho_{a^+_{k},k} $.

Finally, $T_{\av}(\psi(t)) \geqslant T_{\av}^{\tilde\av}(\psi(t)) \geqslant \epsilon \tilde{T}_{\tilde\av}(t) \geqslant 1$, and therefore $b_{a_k, k}(\psi(t))$ and $\hat\rho_{a_k, k}(\psi(t))$ are properly defined for any position $k\in[K]$.

Then, by Pinsker's inequality and the fact that $\psi(t)\leqslant t$, $\tilde{T}_{\tilde\av}(s)$ is non-decreasing in $s$, and $T_{\av}(\psi(t)) \geqslant \epsilon \tilde{T}_{\tilde\av}(t) $, 
\begin{align*}
\sum_{k} b_{a_k, k}(\psi(t)) - \sum_{k}  b_{a^+_k, k}(\psi(t))
&= \sum_{k\in\Kc} b_{a_k, k}(\psi(t)) - b_{a^+_k, k}(\psi(t))
\\
&\leqslant \sum_{k\in\Kc} \hat\rho_{a_k, k}(\psi(t)) +  \sqrt{\frac{\log(\tilde{T}_{\tilde\av}(\psi(t))+1)+3\log(\log(\tilde{T}_{\tilde\av}(\psi(t))+1))}{2T_{\av}(\psi(t))}} - b_{a^+_k, k}(\psi(t))
\\
&< \sum_{k\in\Kc} \rho_{a_k, k} + \frac{\delta}{8} + \sqrt{\frac{\log(\tilde{T}_{\tilde\av}(t)+1)+3\log(\log(\tilde{T}_{\tilde\av}(t)+1))}{2\epsilon \tilde{T}_{\tilde\av}(t)}} - \rho_{a^+_k, k}
\\
&\leqslant \sum_{k\in\Kc} \rho_{a_k, k} + \frac{\delta}{8} + \frac{\delta}{8} - \rho_{a^+_k, k}
\\
&\leqslant \sum_k \rho_{a_k, k} - \sum_k \rho_{a^+_k, k}  + |\Kc| \cdot2\frac{\delta}{8}
\\
&\leqslant -\delta  + 8\frac{\delta}{8}
\\
&=0,
\end{align*}
which contradicts the fact that $\av$ is played at iteration $\psi(t)$. So $\psi(t) \in D \cup E \cup F$.

Overall, for any $t\in B_{t_0}^T$,  $\psi(t) \in D \cup E \cup F$. So, $ B_{t_0}^T \subseteq  \bigcup_{n\in D \cup E \cup F} B_{t_0}^T\cap\left\{t\in [T]: \psi(t)=n \right\}$. Let $n$ be in $D \cup E \cup F$. For any $t$ in $B_{t_0}^T\cap\left\{t\in [T]: \psi(t)=n \right\}$, $T_{\av(n)}^{\tilde\av}(n) = \lceil\epsilon \tilde{T}_{\tilde\av}(t)\rceil$ and $\tilde{T}_{\tilde\av}(t+1)=\tilde{T}_{\tilde\av}(t)+1$. So $|B_{t_0}^T\cap\left\{t\in [T]: \psi(t)=n \right\}| < 1/\epsilon+1$.
Overall,
$$\EE\left[|B|\right]
\leqslant t_0 + \EE\left[|B_{t_0}^T|\right]
\leqslant t_0 + \left(1/\epsilon+1\right)(\EE\left[|D|\right]+\EE\left[|E|\right]+\EE\left[|F|\right]).$$

It remains to upper-bound $\EE\left[|D|\right]$, $\EE\left[|E|\right]$, and $\EE\left[|F|\right]$ to conclude the proof.

\paragraph{Bound on $\EE\left[|D|\right]$}
The upper-bound on $\EE\left[|D|\right]$ is obtained with the same strategy as the last step in the proof of the upper-bound on $\EE\left[|A_{\av^+}|\right]$. Let $ \av$ be a recommendation in $\Nc\cup\{\tilde\av\}\setminus\Nc^+$, and $k \in [K]$ be a position. $D_{\av,k} \subseteq \bigcup_{s\in \NN} \Lambda_{\av,k}(s)$, where $\Lambda_{\av,k}(s) \defeq \{t\in D_{\av,k} : T_{\av}(t)=s\}$. $|\Lambda_{\av,k}(s)| \leqslant 1$ as  $T_{\av}(t)$ increases for each $t\in D_{\av,k}$. Note that for each $s\in \NN$ and $n\in \Lambda_{\av,k}(s)$, $T_{a_k, k}(n) \geqslant T_{\av}(n)=s$. Then, by Lemma \ref{lem:B1}

\begin{align*}
    \EE\left[|D_{\av,k}|\right]
    &\leq\EE\left[\sum_{t=1}^T \ind\{t \in D_{\av,k}\}\right]\\
    & = \EE\left[\sum_{t=1}^T \ind\left\{t \in D_{\av,k},  |\hat\rho_{a_k, k}(t) - \rho_{a_k, k}| \geqslant \frac{\delta}{8} \right\}\right]\\
    & \leqslant \frac{64}{\delta^2}
\end{align*}
Hence, $\EE\left[|D|\right] \leq
\sum_{(\av,k) \in (\Nc\cup\{\tilde\av\}\setminus\Nc^+)\times[K]}\EE\left[|D_{\av,k}|\right]
\leqslant \frac{64(N+1)K}{\delta^2}$.



\paragraph{Bound on $\EE\left[|E|\right]$}


By Theorem 10 of \cite{Garivier2011}, $\EE\left[|E_{\av^+,k}|\right] = O(\log(\log(T)))$, so 
$\EE\left[|E|\right]
\leqslant \sum_{(\av^+,k)\in \Nc^+\times [K]}
\EE\left[|E_{\av^+,k}|\right] = O(|\Nc^+|K\log(\log(T)))$.


\paragraph{Bound on $\EE\left[|F|\right]$}

By Lemma \ref{lem:badordering}, $\EE\left[|F|\right] = \EE\left[\sum_{t=1}^T\ind\left\{\tilde\av(t)=\tilde\av,\\ \tilde\piv(t)\notin\Pi_\rhov\left(\tilde\av\right) \right\}\right]
= \OO\left(1\right).$

Overall $\EE\left[\ind\{\tilde\av(t)=\tilde\av\}\right] \leqslant
\frac{|\Kc^+|}{\epsilon}
+ \frac{8|\Kc^+|^3|\Nc^+|}{\epsilon\delta^2}
+ t_0
+ \left(\frac{1}{\epsilon}+1\right)\frac{64(N+1)K}{\delta^2}
+ \OO\left(\frac{|\Nc^+|K}{\epsilon}\log\log T\right)
+\OO(1)
= \OO\left(\frac{|\Nc^+|K}{\epsilon}\log\log T\right)$, which concludes the proof.
\end{proof}



\section{Proof of Lemma \ref{lem:badordering} (Upper-bound on the Number of Iterations of \ouralgo{} for which $\tilde\piv(t) \notin \Pi_\rhov(\tilde\av)$)}\label{app:badordering}

\begin{proof}[Proof of Theorem \ref{lem:badordering}]
Let $\tilde\av$ be a $K$-permutation of $L$ items. If $\Pi_\rhov\left(\tilde\av\right)$ contains all the permutations of $K$ elements, the set $\left\{t:\tilde\av(t)=\tilde\av, \tilde\piv(t)\notin \Pi_\rhov\left(\tilde\av\right)\right\}$ is empty.

Otherwise, let denote $\delta$ the smallest non-zero gap between the probability of click at position $k$ and the probability of click at position $k'\neq k$: $\delta\defeq\min \left\{\rho_{\tilde{a}_k,k}-\rho_{\tilde{a}_{k'},k'} : (k,k')\in[K]^2, \rho_{\tilde{a}_k,k}-\rho_{\tilde{a}_{k'},k'}>0\right\}$. The gap $\delta$ is the minimum on a finite set, so $\delta>0$.

By definition of $\tilde\pi(t)$,
$\hat\rho_{\tilde{a}_{\tilde\pi_1(t)}(t),\tilde\pi_1(t)}(t) \geqslant \hat\rho_{\tilde{a}_{\tilde\pi_2(t)}(t),\tilde\pi_2(t)}(t) \geqslant \dots \geqslant \hat\rho_{\tilde{a}_{\tilde\pi_K(t)}(t),\tilde\pi_K(t)}(t),$
so,
\begin{align*}
    \left\{t:\tilde\av(t)=\tilde\av, \tilde\piv(t)\notin\Pi_\rhov\left(\tilde\av\right)\right\}
    &= \bigcup_{\tilde\piv\in\perm_K^K}\bigcup_{k\in[K-1]}
    \left\{t:\tilde\av(t)=\tilde\av, \tilde\piv(t)=\tilde\piv,
    \rho_{\tilde{a}_{\tilde\pi_k}, \tilde\pi_k} < \rho_{\tilde{a}_{\tilde\pi_{k+1}}, \tilde\pi_{k+1}}\right\}
    \\
    &\subseteq \bigcup_{\tilde\piv\in\perm_K^K}\bigcup_{k\in[K-1]}
    \left\{t:\tilde\av(t)=\tilde\av, \tilde\piv(t)=\tilde\piv, 
    \substack{
    |\hat\rho_{\tilde{a}_{\tilde\pi_k}, \tilde\pi_k}(t)
        - \rho_{\tilde{a}_{\tilde\pi_k}, \tilde\pi_k}| > \frac{\delta}{2}\\
    \text{ or }|\hat\rho_{\tilde{a}_{\tilde\pi_{k+1}}, \tilde\pi_{k+1}}(t)
        - \rho_{\tilde{a}_{\tilde\pi_{k+1}}, \tilde\pi_{k+1}}| > \frac{\delta}{2}
    }
    \right\}
    \\
    &= \bigcup_{\tilde\piv\in\perm_K^K}\bigcup_{k\in[K]} \Lambda_{\tilde\piv,k},
\end{align*}
with
$\Lambda_{\tilde\piv,k} \defeq \left\{t:\tilde\av(t)=\tilde\av, \tilde\piv(t)=\tilde\piv, 
    |\hat\rho_{\tilde{a}_{\tilde\pi_k}, \tilde\pi_k}(t)
        - \rho_{\tilde{a}_{\tilde\pi_k}, \tilde\pi_k}| > \frac{\delta}{2}\right\},$
for any ranking of positions $\tilde\piv\in\perm_K^L$ and any rank $k\in [K]$.

Let $\tilde\piv\in\perm_K^L$ be a ranking of positions, and $k\in[K]$ be a rank.
$\Lambda_{\tilde\piv,k} \subseteq \bigcup_{s\in\NN}\Lambda_{\tilde\piv,k}(s)$, with $\Lambda_{\tilde\piv,k}(s) \defeq \{t\in \Lambda_{\tilde\piv,k}: \tilde{T}_{\tilde\av}(t) = s\}$. $|\Lambda_{\tilde\piv,k}(s)| \leqslant 1$ as $\tilde{T}_{\tilde\av}(t)$ increases for each $t\in \Lambda_{\tilde\piv,k}$.  Note that for each $s\in \NN$ and $n \in \Lambda_{\tilde\piv,k}(s)$, $T_{\tilde{a}_{\tilde\pi_k}, \tilde\pi_k}(n) \geqslant T_{\tilde\av}(n)\geqslant \tilde{T}_{\tilde\av}(n)/L=s/L$. Then, by Lemma \ref{lem:B1}
\begin{align*}
\EE\left[|\Lambda_{\tilde\piv,k}|\right]
&=\EE\left[\sum_{t=1}^T \ind\{t \in \Lambda_{\tilde\piv,k}\}\right]\\
& = \EE\left[\sum_{t=1}^T \ind\left\{t \in \Lambda_{\tilde\piv,k}, |\hat\rho_{\tilde{a}_{\tilde\pi_k}, \tilde\pi_k}(t) - \rho_{\tilde{a}_{\tilde\pi_k}, \tilde\pi_k}| > \frac{\delta}{2} \right\}\right]\\
& \leqslant \frac{4L}{\delta^2}
\end{align*}

Hence,
\begin{align*}
\EE\left[\sum_{t=1}^T\ind\{\tilde\av(t)=\tilde\av, \tilde\piv(t)\notin\Pi_\rhov\left(\tilde\av\right) \}\right]
&\leqslant \sum_{\tilde\piv\in\perm_K^K}\sum_{k\in[K]} \EE\left[\Lambda_{\tilde\piv,k}\right]
\\
&\leqslant \frac{4LKK!}{\delta^2}
\\
&= \OO\left(LKK!\right),
\end{align*}
which concludes the proof.

\end{proof}





%\section{Opponent's tuning}
%\subsection{$\epsilon_n$-Greedy's tuning }

%For $\epsilon_n$-Greedy, we use SVD to define the estimation $(\hat\thetav, \hat\kappav)$ of parameters  $(\thetav, \kappav)$.We infere  the \emph{Maximum A Posteriori} (MAP) value for $(\thetav, \kappav)$ given the collected data with an expectation-maximisation (EM) approach \cite{Chuklin2015} and a SVD. We did compare the cumulative regret obtained using SVD and using EM with the Pyclick implementation \cite{Chuklin2015} for $\epsilon_n$-Greedy algorithm. Both inference processes led to recommendations with similar regret, but the SVD version was about 700 times faster, so we decided to use SVD for all other experiments.
  
%We also have to tune the parameter $c$ of $\epsilon_n$-Greedy. On the one hand, having a $c$ too small prevents the algorithm from enough exploring and forces it to learn wrong values for the parameters $(\thetav, \kappav)$. On the other hand, the greater $c$ is, the more  %$\epsilon_n$-greedy explores and loses positive rewards in the process.
%  Figure \ref{fig:hyperparam_greedy} shows the cumulative regret obtained for each dataset when $c$ takes the values $10^0, 10^1, \dots,$ and  $10^6$. In order to obtain the best result, we pick the best value of $c$ on a per dataset basis: $10^4$ for Yandex settings,$10^{3}$ when $\thetav$ is close to 1, and  $10^{5}$ when $\thetav$ is close to $0$.

   

%\begin{figure}[h!]
%	\begin{minipage}[b]{0.40\linewidth}
%		\centering \includegraphics[scale=0.68]{Graph/xlog_Yandex__eGeeedy_20g_10000000t.pdf}
%		\caption{Yandex}
%		\label{fig:PBMHB_Yandex}
%	\end{minipage}
%	\begin{minipage}[b]{0.30\linewidth}	
%		\centering \includegraphics[scale=0.62]{Graph/xlog_big__eGeeedy_20g_10000000t.pdf}
%		\caption{simulated, $\thetav^+$}
%		\label{fig:PBMHB_big}
%	\end{minipage}
%	\begin{minipage}[b]{0.40\linewidth}
%		\centering \includegraphics[scale=0.68]{Graph/xlog_xxsmall__eGeeedy_20g_10000000t.pdf}
%		\caption{simulated, $\thetav^-$}
%		\label{fig:PBMHB_small}
%	\end{minipage}
%	
%	\begin{minipage}[b]{1.10\linewidth}
%		\centering \includegraphics[scale=0.8]{Graph/eGeeedy_20g_10000000t_legend.pdf}
%	\end{minipage}

%\caption{Cumulative regret w.r.t.  iteration. Impact of the parameter $c$ in $\epsilon_n$-Greedy. The shaded area depicts the standard error of our regret estimates.\label{fig:hyperparam_greedy}}
%\end{figure}   
   

%\subsection{PB-MHB's tuning}

%According to \cite{PBMHB}, PB-MHB's behavior is mostly affected by two to three hyper-parameters: the width $c/\sqrt{t}$ of the Gaussian random-walk steps, the number $m$ of Metropolis-Hastings iterations per recommendation and the starting point of the its Metropolis Hastings'particule. Authors show that the later too parameter mostly influences the efficiency of the algorithm and that by start from the couple $(\tilde\thetav, \tilde\kappav)$ from the previous iteration with $m =1$, only $c$ influences the regret. we show in Figure \ref{fig:hyperparam_PBMHB} that PB-MHB exhibits the smallest regret on every settings as soon as $c>100$ but to prevent from lost in the regret as in Figure \ref{fig:PBMHB_big} and respect \cite{PBMHB} recommendation we used $c=1000$  .
   


%\begin{figure}[h!]
%	\begin{minipage}[b]{0.40\linewidth}
%%		\centering \includegraphics[scale=0.68]{Graph/PB_MHB_Yandex_tune_c_TGRW.pdf}
%		\caption{Yandex}
%	\end{minipage}
%	\begin{minipage}[b]{0.30\linewidth}	
%		\centering \includegraphics[scale=0.66]{Graph/PB_MHB_big_tune_c_TGRW.pdf}
%		\caption{simulated, $\thetav^+$}
%%	\begin{minipage}[b]{0.40\linewidth}
%		\centering \includegraphics[scale=0.68]{Graph/PB_MHB_xxsmall_tune_c_TGRW.pdf}
%		\caption{simulated, $\thetav^-$}
%	\end{minipage}
%	
%	\begin{minipage}[b]{1.10\linewidth}
%		\centering \includegraphics[scale=0.8]{Graph/ICML_legend_tunePBMHB.pdf}
%	\end{minipage}
%
%\caption{Cumulative regret w.r.t.  iteration. Impact of the parameter $c$ in PB-MHB. The shaded area depicts the standard error of our regret %estimates.\label{fig:hyperparam_PBMHB}}
%\end{figure}   
   




\begin{algorithm}[tb]
\caption{KL-ComUCB1 (generic version)}\label{alg:KL-ComUCB1_generic}
\begin{algorithmic}
\REQUIRE set of elements $E$, set of arms $\Ac$
\STATE $t\gets 1$
\WHILE{$\{e\in E:T_e(t)=0\} \neq \varnothing$}
\STATE $\tilde{E} \gets \{e\in E: T_e(t)=0\}$
\STATE $\tilde{\Ac} \gets \{\av\in\Ac :  \av \cap \tilde{E}\neq\varnothing\}$
\STATE recommend $\displaystyle\av(t) = \argmax_{\av \in \tilde\Ac}
\sum_{e\in \av}b_{e}(t)$
\STATE observe the weights $\left[w_e(t) : e\in\av\right]$
\STATE $t\gets t+1$
\ENDWHILE
\STATE $t_0\gets t$
\FOR{$t =  t_0, t_0+1, \dots$}
\STATE recommend $\displaystyle\av(t) = \argmax_{\av \in \Ac}
\sum_{e\in \av}b_{e}(t)$  
\STATE observe the weights $\left[w_e(t) : e\in\av\right]$
\ENDFOR
\end{algorithmic}
\end{algorithm}


\section{KL-CombUCB and its Application to PBM Setting} \label{app:KL-Comb_to_PBM}
In this section we first define the generic combinatorial semi-bandit algorithm KL-CombUCB and we compare two upper-bounds on its regret. Then, we present the application of KL-CombUCB to PBM setting and discuss its relation to \ouralgo{}.

\subsection{KL-CombUCB for Generic Setting}

CombUCB1 \cite{Kveton2015CombUCB} is a bandit algorithm handling the following combinatorial setting. Let $E$ be a set of elements and $\Ac\subseteq\{0,1\}^E$ be a set of arms, where each arm $\av$ is a subset of $E$.
Following the terminology used in \cite{Kveton2015CombUCB}, $E$ is the \emph{ground set} and $\Ac$ the \emph{feasible set}. 
At each iteration, the bandit algorithm chooses a subset of elements $\av\in\Ac$ and receives the reward $\sum_{e \in \av} w_e$, where $\wv$ is an independent draw of a distribution $\nu$ on $[0,1]^E$. Given these assumptions, CombUCB1 chooses an arm $\av(t)$ at each iteration, aiming at minimizing the total regret defined as usual.

%The rest of the exposition requires more notations. 
We denote $\rho_e\defeq\EE_{\wv\sim \nu}\left[w_e\right]$ the expected reward associated to element $e$,
$\mu_\av\defeq \EE_{\wv\sim \nu}\left[\sum_{e \in \av} w_e\right]=\sum_{e\in\av}\rho_e$ the expected reward when choosing the arm $\av\in\Ac$,
and $\mu^*\defeq\max_{\av\in \Ac}\mu_\av$ the best expected reward.
We also denote $\Delta_\av \defeq \mu^*-\mu_\av$ the gap between the best expected reward and the reward of an arm $\av$,
and $\Delta_{min} \defeq \min_{\av \in\Ac:\Delta_\av>0} \Delta_\av$ the smallest gap of a suboptimal arm.
Finally,
$K\defeq\max_{\av\in\Ac}|\av|$ denotes the maximum size of an arm (meaning the maximum number of chosen elements),
$K_\av \defeq \min_{\av^*\in\Ac: \mu_{\av^*}=\mu^*} |\av\setminus\av^*|$ is the smallest number of elements to remove from $\av$ to get an optimal arm,
and $K_{max}\defeq\max_{\av \in\Ac: \mu_\av\neq\mu^*} K_\av$ is its lager value.


In our paper, we use the Kullback-Leibler variation of CombUCB1 which chooses the arm based on the index $b_e(t)$ (defined hereafter) instead of the usual confidence upper-bound derived from the Hoeffding’s inequality. The corresponding algorithm (KL-CombUCB) also assumes that the weight-vector $\wv(t)$ is in $\{0,1\}^E$. KL-CombUCB is depicted by Algorithm \ref{alg:KL-ComUCB1_generic} which uses the following notations. At each iteration $t$,
we denote 
$$\hat\rho_e(t) \defeq \frac{1}{T_e(t)}\sum_{s = 1}^{t-1} \ind\{e \in \av(s)\}w_e(s)$$
the average number of clicks obtained by the element $e$, where
$$T_e(t) \defeq \sum_{s = 1}^{t-1} \ind\{e \in \av(s)\}$$
is the number of times element $e$ has been selected; $\hat\rho_e(t)\defeq0$ when $T_e(t)=0$.
The statistics $\hat\rho_e(t)$ are paired with their respective \emph{indices} $$b_e(t) \defeq f\left(\hat\rho_e(t), T_e(t), t\right),$$
where
$f(\hat\rho, s, t)$ stands for $$\sup \{p\in[\hat\rho,1]: s\times\KL(\hat{\rho}, p) \leq \log (t) + 3 \log(\log (t))\},$$
with
$$\KL(p,q) \defeq p \log \left(\frac{p}{q}\right) + (1-p)\log \left(\frac{1 - p}{1 - q}\right)$$
the \emph{Kullback-Leibler divergence} from a Bernoulli distribution of mean $p$ to a Bernoulli distribution of mean $q$;
$f(\hat\rho, s, t) \defeq 1$ when $\hat{\rho}=1$, $s=0$, or $t=0$. 

\citeauthor{Kveton2015CombUCB} prove that the regret of CombUCB1 is upper-bounded by $\OO\left(|E|K/\Delta_{min}\log T\right)$, and a similar proof would lead to the same upper-bound for KL-CombUCB. In our paper we prove in Theorem \ref{theo:good_leader} a completely different regret upper-bound for KL-CombUCB: $\OO\left(|\Ac|K_{max}^2/\Delta_{min}\log T\right)$. For most combinatorial bandit settings, this new bound is useless since $|\Ac| \gg |E|$, and $K_{max} \approx K$. However, the analysis of \ouralgo{} involves an application of KL-CombUCB to a setting where the new bound is smaller than the standard one as $|\Ac| = |E|-1$ and $K_{max}=2$.


\begin{algorithm}[tb]
\caption{KL-ComUCB1 (applied to PBM)}\label{alg:KL-ComUCB1}
\begin{algorithmic}
\REQUIRE number of items $L$, number of positions $K$
\FOR{$t =  1, 2, \dots, L$}
\STATE recommend $\displaystyle\av(t) = \left(((t -1)\% L) + 1, (t\% L) + 1, \dots, ((t +K-2) \% L) + 1\right)$  
\STATE observe the clicks-vector $\cv(t)$
\ENDFOR
\FOR{$t =  L+1, L+2, \dots$}
\STATE recommend $\displaystyle\av(t) = \argmax_{\av \in \perm_K^L}
\sum_{k=1}^Kb_{a_k, k}(t)$  
\STATE observe the clicks-vector $\cv(t)$
\ENDFOR
\end{algorithmic}
\end{algorithm}

\subsection{KL-CombUCB Applied to PBM Setting}


In the experiments (Section 6), we apply KL-CombUCB to PBM bandit setting by choosing the \emph{ground set} $E = [L]\times[K]$, the \emph{feasible set} $\Theta=\{\{(a_k,k): k \in [K]\}:\av\in\perm_K^L\}$, and the \emph{expected weights} $\rho_{(i,k)}=\theta_i\kappa_k$ for any ``element" $(i,k)\in E$. Note that the observed weights of the generic setting correspond to the clicks-vector in the PBM setting. 

The corresponding algorithm, depicted by Algorithm \ref{alg:KL-ComUCB1}, recommends at each iteration $t$ the best permutation given the indices $b_{i,k}(t)$ defined for \ouralgo{}. This optimization problem
is a \emph{linear sum assignment problem} which is solvable in $\OO\left(K^2(L+\log K)\right)$ time \cite{Ramshaw2012}. Note the close relationship with \ouralgo{}:
\begin{itemize}
    \item both algorithms solve a linear sum assignment problem, they only differ from the metric to optimize: $\sum_{k=1}^K\hat\rho_{a_k, k}(t)$ for \ouralgo{} vs. $\sum_{k=1}^Kb_{a_k, k}(t)$ for KL-CombUCB;
    \item both algorithms recommend the best permutation $\av$ regarding  $\sum_{k=1}^Kb_{a_k, k}(t)$, they only differ from the considered set of permutations:  $\{\tilde\av(t)\}\cup\Nc_{\tilde\piv(t)}\left(\tilde\av(t)\right)$ for \ouralgo{} vs. $\perm_K^L$ for KL-CombUCB.
\end{itemize}
 
By considering a larger set of permutations, KL-ComUCB1 suffers a $\OO(LK^2/\Delta_{min}\log T)$ regret (by applying \cite{Kveton2015CombUCB} bound), which is higher than the upper-bound on the regret of \ouralgo{} by a factor $K^2$. 




\section{\ouralgofull{}: OSUB on a Static Graph}\label{app:fgrab}

\begin{algorithm}[tb]
\caption{\ouralgofull{}: \ouralgofulllong{}}\label{alg:S-GRAB}
\begin{algorithmic}
\REQUIRE number of items $L$, number of positions $K$
\STATE $\gamma\gets K(2L-K-1)/2$
\FOR{$t =  1, 2, \dots$}
\STATE $\displaystyle\tilde\av(t) \gets \argmax_{\av \in \perm_K^L}
\sum_{k=1}^K \hat\rho_{a_k,k}(t)$
\STATE
$\displaystyle
\text{recommend }
\av(t) =\begin{cases}
 \tilde\av(t)
 & \text{, if } \frac{\Tilde{T}_{\tilde\av(t)}(t)}{\gamma+1} \in \mathds{N}, \\
 \displaystyle \argmax_{\av \in \{\tilde\av(t)\}\cup\Nc_G(\tilde\av(t))}
 \sum_{k=1}^K b_{a_k, k}(t)
% -
 %\sum_{k=1}^K
% b_{\tilde{a}_k(t), k}
& \text{, otherwise}
\end{cases} $
\\
where $\Nc_G(\av) = \left\{\av \circ (k,k'):  k,k' \in [K]^2, k>k'\right\} \cup
\left\{\av[k := i]: k \in [K], i \in [L]\setminus\av([K])\right\}$
\STATE observe the clicks vector $\cv(t)$
\ENDFOR
\end{algorithmic}
\end{algorithm}


The algorithm \ouralgofull{}, depicted in Algorithm \ref{alg:S-GRAB}, is similar to \ouralgo{} except that it explores a static graph $G=(E, V)$ defined by
\begin{align*}
V&\defeq\perm_K^L,\\
E &\defeq
\left\{(\av, \av \circ (k,k')):  k,k' \in [K]^2, k>k'\right\}
\cup\left\{(\av, \av[k:= i]):  k\in [K], i \in [L]\setminus\av([K])\right\}.
\end{align*}


This graph is chosen to ensure that with PBM setting any sub-optimal recommendation has a strictly better recommendation in its neighborhood given $G$. This graph is fixed and does not require the knowledge of a mapping $\cal P$, but its degree is also about $K$ times larger than the degree of the graphs handled by \ouralgo{}. 

As for \ouralgo{}, any recommendation in the neighborhood of the leader given $G$ differs with the leader at, at most two positions. Therefore a proof similar to the one of Theorem \ref{theo:osrubpbm} ensures that \ouralgofull{}'s regret is upper-bounded by $\OO\left(LK/\Delta_{min}\log T\right)$. This regret upper-bound is higher than \ouralgo{}'s one by a factor $K$ due to the larger size of the considered neighborhoods. However, this regret remains smaller than KL-CombUCB's one by a factor $K$ thanks to the bounded number of differences between the leader and the arm played.

%\bibliography{bib.bib}
%\bibliographystyle{icml2021}

